The regularity theory for the Mumford-Shah functional on the plane

The aim of these notes is to give a complete self-contained account of the current state of the art in the regularity for planar minimizers and critical points of the Mumford-Shah functional.

==> vecchio_capitolo_6.tex <==
\section{Parti gia' scritte da Matteo}

On the other hand it is not difficult to see that, if the Mumford-Shah conjecture holds, then $\nabla u\in L^p_{loc}$ 
for all $p<4$ (cf. with \cite[Proposition~6.3]{AFH} under $C^{1,1}$ 
regularity assumptions on $K$, see also 
Theorem~\ref{t:summability}). 

According to Ambrosio, Fusco and Hutchinson's theory, the higher integrability of the gradient can be translated into an estimate on the Hausdorff dimension of the 
singular set $\Sigma$ of $K$ (see \cite[Corollary 5.7]{AFH}) that improves 
upon the conclusion of item (i) in Theorem~\ref{t:structure} 


In addition, we shall show that $\Sigma^{(1)}\subset K^r$, that (regular) loose ends belong to $\Sigma^{(2)}\cap K^r$, and that irregular terminal 
points, provided that they exist, belong to $\Sigma^{(2)}\cap K^i$.

In this section we shall prove some estimates on the size of $\Sigma$.
A first breakthrough in this direction has been obtained by Ambrosio, Fusco and Hutchinson \cite{AFH}\footnote{The theory developed in \cite{AFH} holds more generally in a higher dimensional setting with suitable changes in the statements.}.
\begin{theorem}%[Ambrosio, Fusco and Hutchinson, \cite{AFH}]
\label{t:AFH2}
Let $(K,u)$ be a restricted, absolute, or generalized global minimizer of $E_\param$ in $\Omega$, then
\[
\dimh \Sigma^{(1)}=0\, . %\leq n-2.
\]
\end{theorem}
Actually, the set $\Sigma^{(1)}$ turns out to be countable (cf. Corollary~\ref{c:tj} below).

Moreover, in the same paper \cite{AFH}, Ambrosio, Fusco and Hutchinson investigated the 
connection between the higher integrability of $\nabla u$ and the Mumford-Shah conjecture. 
If the conjecture is true, then $\nabla u\in L^p_{loc}$ 
for all $p<4$ (cf. with \cite[Proposition~6.3]{AFH} under $C^{1,1}$ 
regularity assumptions on $K$, see also 
Theorem~\ref{t:summability}). 
It was indeed conjectured by De Giorgi (in all space dimensions) that 
$\nabla u\in L^p_{loc}$ for all $p<4$ (cf. with \cite[conjecture 1]{DG}).
So far only a first step into this direction has been established. 
\begin{theorem}\label{t:hi}
There is $p>2$ such that $\nabla u\in L^p_{\mathrm{loc}}(\Omega)$ for all
$(K,u)$ either restricted, or absolute, or generalized global minimizer of 
$E_\param$ in $\Omega$, and for all open sets $\Omega\subseteq\R^2$.
\end{theorem}
Theorem~\ref{t:hi} has been proven first by De~Lellis and Focardi in \cite{DLF13} in $2$d (cf. Section~\ref{ss:reverse holder}). Shortly after 
De~Philippis and Figalli established the result without any dimensional limitation in 
\cite{DePFig14} (cf. Section~\ref{ss:porosity}). 
The exponent $p$ in both papers is not explicitly computed despite potentially this could be done. In any case it would lead only to a slight gain in the integrability exponent.

According to Ambrosio, Fusco and Hutchinson's theory, the higher integrability of the gradient can be translated into an estimate on the Hausdorff dimension of the 
singular set $\Sigma$ of $K$ (see \cite[Corollary 5.7]{AFH}) that improves 
upon the conclusion of item (i) in Theorem~\ref{t:structure} 
\begin{theorem}%[Ambrosio, Fusco and Hutchinson \cite{AFH}]
\label{t:AFH1}
Let $(K,u)$ be a restricted, absolute, or generalized global minimizer of $E_\param$ in $\Omega$ be such that $\nabla u\in L^p_{{loc}}(\Omega)$ for some $p>2$, then 
\begin{equation}\label{e:stimaSigmau}
\mathrm{dim}_\HH\Sigma\leq 2-\frac p2\in(0,1)\,.
%\max\{n-2,n-\sfrac p2\}\in(0,n-1).
\end{equation}
 \end{theorem}
 % Given Theorems~\ref{t:AFH2} and \ref{t:hi} for granted, Theorem~\ref{t:AFH1} is a simple consequence 
%of soft measure theoretic arguments. We shall establish Theorem~\ref{t:AFH2} in Section~\ref{ss:cpt}. 
%Instead, here we prove Theorem~\ref{t:AFH1} to underline the role of the higher 
%integrability that, in turn, shall be established in Sections~\ref{ss:reverse holder} and \ref{ss:porosity} following two different paths. 
\
\begin{proof}%[Proof of Theorem~\ref{t:AFH1}]
Suppose that $|\nabla u|\in L^p_{loc}(\Omega)$ for some $p>2$, then for all $s\in(2-\sfrac p2,1)$ 
the set 
\[
\Lambda_s:=\left\{x\in\Omega:\,
\limsup_{r\to 0}r^{-s}\int_{B_r(x)}|\nabla u|^p=\infty\right\}
\]
satisfies $\HH^s(\Lambda_s)=0$ by elementary density estimates for the Radon measure defined on any subset $E\subseteq\Omega$ by
\[
\mu(E):=\int_E|\nabla u|^p\,.
\]
Indeed, Theorem~\ref{t:dlb} and the density estimates in 
\cite[Theorem~2.56]{AFP00} give that
\[
\frac\e2\,\HH^s(\Lambda_s)\leq \mu(\Lambda_s)\leq\mu(\Omega)<\infty. 
\]
Therefore, $\mathcal{L}^2(\Lambda_s)=0$.
In turn plugging this piece of 
information in the previous inequality gives $\mu(\Lambda_s)=\HH^s(\Lambda_s)=0$. 

Hence, if we rewrite $\Sigma$ as the disjoint union of $\Sigma\cap \Lambda_s$
and of $\Sigma\setminus\Lambda_s$, we deduce $\HH^s(\Sigma\cap \Lambda_s)=0$ 
and thus $\mathrm{dim}_\HH(\Sigma\cap \Lambda_s)\leq s$.
 Furthermore, it is easy to prove that $\Sigma\setminus\Lambda_s\subseteq\Sigma^{(1)}$. 
If $x\in\Sigma\setminus\Lambda_s$ by the higher integrability 
and H\"older inequality it follows that
\[
d(x,r)=r^{-1}\int_{B_r(x)}|\nabla u|^2
\leq\, \pi^{1-\frac 2p}\,r^{\frac 2p(s-2+\frac p2)}
\left(r^{-s}\int_{B_r(x)}|\nabla u|^p\right)^{\frac 2p}
\stackrel{r\downarrow 0^+}{\longrightarrow}0,
\]
as $s>2-\sfrac p2$. 
Theorem~\ref{t:AFH2} yields
$\mathrm{dim}_\HH(\Sigma\setminus \Lambda_s)=0$.

In conclusion, we infer that for all $s\in(2-\sfrac p2,1)$
\[
\mathrm{dim}_\HH\Sigma=\max\{\mathrm{dim}_\HH(\Sigma\cap \Lambda_s), 
\mathrm{dim}_\HH(\Sigma\setminus\Lambda_s)\}= s,
\] 
and the conclusion follows by letting $s\downarrow(2-\sfrac p2)$.
\end{proof}

The estimate $\mathrm{dim}_\HH\Sigma<1$ has been obtained first by David \cite{david1996} using the \emph{porosity} of \index{porosity@porosity}
$\Omega\cap K$ (cf. Theorem~\ref{t:RMS} below, and 
Rigot \cite{Rig00}, Maddalena and Solimini \cite{MadSol01} in higher dimensions). 
Despite this, it was not quantitative and unrelated to the higher integrability property 
of the gradient. 

We conclude this introductory section to the topic with 
a couple of remarks:
\begin{itemize}
\item[(i)] a first trivial motivation for the upper bound $p<4$ is that the right hand side in the estimate \eqref{e:stimaSigmau} has to be positive. More importantly, cracktips show that $4$ is the best possible exponent occurring in general. Indeed, 
consider the prototype cracktip minimizer (Bonnet and David \cite{bonnetdavid2001}) 
\begin{equation}\label{e:uct}
u_{ct}(r,\theta)=\sqrt{\frac 2\pi r}\,\cos(\frac\theta2),\qquad K_{ct}=[0,\infty)
\end{equation}
for $\theta\in(0,2\pi)$ and $r>0$. It is easy to check that 
$|\nabla u_{ct}|\in L^p\setminus L^4_{loc}(\R^2\setminus K_{ct})$, for all $p<4$;

\item[(ii)] in addition, the validity of the higher integrability property
for every $p<4$ and  \eqref{e:stimaSigmau} would then imply that $\mathrm{dim}_\HH\Sigma=0$. 
As we shall prove below, the sharper higher integrability stated in Theorem~\ref{t:summability} is actually equivalent to it.
\end{itemize}


\subsection{An energetic characterization of the Mumford-Shah conjecture}\label{ss:enconj}

Let us go back to the upper bound $p<4$ in the higher integrability result. 
We consider again the cracktip function 
$u_{ct}$ in \eqref{e:uct}. 
As recalled in the previous section $\nabla u_{ct}\in L^p\setminus L^4_{loc}(\R^2\setminus K_{ct})$ 
for all $p<4$. Actually, one can easily prove that 
$|\nabla u_{ct}|\in L^{4,\infty}_{{loc}}(\R^2\setminus K_{ct})$\footnote{We recall that $f\in L^{4,\infty}_{{loc}}(U)$, $U\subset\R^2$ open, if for all $U'\subset\hskip-0.125cm\subset U$ there exists $K=K(U')>0$ 
such that 
\[
 \mathcal{L}^2\left(\{x\in U':\,|f(x)|>\lambda\}\right)\leq K\lambda^{-4}\quad\text{ for all }
\lambda>0.
\]}.
As a side effect of the considerations in \cite{DLF13} and \cite{DFG}, 
one deduces the energetic characterization of the Mumford-Shah conjecture 
stated in Theorem~\ref{t:summability}. %(see \cite[Proposition~1.3]{DFG}). 
%Indeed, the validity of the latter  
%is equivalent to a sharp integrability property of the gradient of the minimizers.
%We recall the statement here for the readers' convenience
%\begin{theorem}\label{t:MSconj}
%Let $(K,u)$ be a restricted, absolute, or generalized global minimizer of $E_\param$ in $\Omega$. The set $K^i$ is empty if and only if $\nabla u \in L^{4,\infty}_{loc}$.
%If $\Omega\subseteq\R^2$, the Mumford-Shah conjecture is true for $u\in\MM(\Omega)$
%if and only if $|\nabla u|\in L^{4,\infty}_{loc}(\Omega)$. 
%\end{theorem}
A key tool for the proof of Theorem~\ref{t:summability} is the following preliminary observation.
\begin{lemma} 
Let $f\in L^{4,\infty}_{loc}(\Omega)$, $\Omega\subseteq\R^2$, then for all $\e>0$ the set
\begin{equation}\label{e:ctip}\
D_\e:=\left\{x\in\Omega:\,\liminf_r\frac 1r\int_{B_r(x)}f^2(y)\ge\e\right\}
\end{equation}
is locally finite.
\end{lemma}
\begin{proof}
We shall show in what follows that if $f\in L^{4,\infty}(\Omega)$ then $D_\e$
is finite, an obvious localization argument then proves the general case.

Let $\e>0$ and consider the set $D_\e$ in \eqref{e:ctip} above.
First note that, for any $B_r (x)\subset \Omega$ and any $\lambda>0$ we have the estimate
\begin{align}\label{e:stimasublev}
\int_{\{y\in B_r(x):\,|f(y)|\geq \lambda\}}f^2(y)&\leq
\int_{\{y\in\Omega:\,|f(y)|\geq \lambda\}}f^2(y)\notag\\
&=2\int_\lambda^{\infty}t\, \mathcal{L}^2\left(\{y\in\Omega:\,|f(y)|\geq t\}\right)dt
\leq\int_\lambda^{\infty}\frac{2K}{t^3}dt=\frac K{\lambda^2}.
\end{align}
If $x\in D_\e$ and $r>0$ satisfy 
\begin{equation}\label{e:stimamisura}
\int_{B_r(x)}f^2(y)\geq \frac \e2 r,
\end{equation}
choosing $\lambda=2(K/r\e)^{1/2}$ in \eqref{e:stimasublev} we conclude 
\begin{equation}\label{e:stimasuplev}
\int_{\{y\in B_r(x):\,|f(y)|<\,2( \frac K{r\e})^{1/2}\}}f^2(y)\geq
%\frac \e2 r-\frac \e6 r\geq
\frac \e4 r.
\end{equation}
Furthermore, the trivial estimate
\[
\int_{\{y\in B_r(x):\,|f(y)|<\lambda\}}f^2(y)<\pi\lambda^2r^2,
\]
implies for $\lambda=(\e/8\pi r)^{1/2}$
\begin{equation}\label{e:stimasublev1}
\int_{\{y\in B_r(x):\,|f(y)|<(\frac \e{8\pi r})^{1/2}\}}f^2(y)<\frac\e 8r.
\end{equation}
By collecting \eqref{e:stimasuplev} and \eqref{e:stimasublev1}
we infer
\[
\int_{\{y\in B_r(x):\,(\frac \e{8\pi r})^{1/2}\leq
|f(y)|<\,2(\frac K{r\e})^{1/2}\}}f^2(y)\geq\frac\e 8r,
\]
that in turn implies
\begin{equation}\label{e:stimafond}
 \mathcal{L}^2\big(\{y\in B_r(x):\,|f(y)|\geq (\frac \e{8\pi r})^{1/2}\}\big)
\geq\frac{\e^2r^2}{32K}.
\end{equation}
Let $\{x_1,\ldots,x_N\}\subseteq D_\e$ and $r>0$ be a radius such 
that the balls $B_r(x_i)\subseteq\Omega$ are disjoint and 
\eqref{e:stimamisura} holds for each $x_i$. Then, from \eqref{e:stimafond} 
and the fact that $f\in L^{4,\infty}(\Omega)$, we infer
\[
N\frac{\e^2r^2}{32K}\leq  \mathcal{L}^2\big(\{y\in\Omega:\,
|f(y)|\geq(\frac \e{8\pi r})^{1/2}\}\big)
\leq\frac {K(8\pi r)^2}{\e^2}\Longrightarrow 
N\leq\frac {2^{11}K^2\pi^2}{\e^4},
\]
and the conclusion follows at once.
\end{proof}

We are now ready to give the proof of Theorem~\ref{t:summability}.
The ``if'' direction is achieved by first proving that $K$ has locally finitely many 
connected components and then invoking the regularity theory developed by Bonnet \cite{B96} and that at regular loose ends established in Theorem~\ref{t:final-cracktip}. 
%together with Theorem~\ref{t:zurrione1}. 
In turn, the proof that the connected components are locally finite 
is a fairly simple application of the $\e$-regularity theory (see Theorem~\ref{t:main}).
Vice versa, the ``only if'' direction is proved by means of Bonnet blow-up analysis
and standard elliptic regularity theory.
\begin{proof}[Proof of Theorem~\ref{t:summability}.]
To prove the direct implication we assume without loss of generality 
that $\Omega=B_R$ for some $R>1$, being the result local. In addition, 
we may also suppose that $K\cap\partial B_1=\{y_1,\ldots,y_M\}$.
Theorem~\ref{t:main} and Theorem~\ref{t:cptness} in Section~\ref{ss:cpt} below yield 
that there exists some $\e_0>0$ such that for all points 
$x\in B_R\setminus D_{\e_0}$ the set $K\cap B_r(x)$ is 
either empty or diffeomorphic to a minimal cone, for some $r>0$. 
In particular, in the latter event $B_r(x)\setminus K$ 
is not connected.

Supposing that $D_{\e_0}\cap B_1=\{x_1, \ldots, x_N\}$, and setting
\[
\Omega_k:= B_{1-1/k}\setminus \bigcup_{i=1}^N B_{1/k}(x_i)\,,
\]
a covering argument and the last remark give that for every 
$x\in\Omega_k\cap K$ there 
is a continuous arc $\gamma_k:[0,1]\to K$ 
with $\gamma_k(0)=x$ and $\gamma_k(1)=y\in\partial\Omega_k$.
Then, the sequence $(\widetilde{\gamma}_k)_{k\in\N}$ of 
reparametrizations of the $\gamma_k$'s by arc length converges 
to some arc $\gamma:[0,1]\to K$ with $\gamma(0)=x$ 
and $\gamma(1)\in\{x_1,\ldots,x_N,y_1,\ldots,y_M\}$.

From this, we deduce that $\overline{B_1}\cap K$ has 
a finite number of connected components.
Bonnet's regularity results \cite[Theorems 1.1 and 1.3]{B96} and Theorem~\ref{t:final-cracktip} then provide the thesis.

We prove next the opposite implication. To this aim we 
consider $\Omega^\prime\subset\hskip-0.125cm\subset\Omega^{\prime\prime}\subset\hskip-0.125cm\subset\Omega$ 
and suppose that $ K\cap\Omega^{\prime\prime}$ is a finite 
union of $C^1$ arcs of finite length. Denote by $\{x_1,\ldots,x_N\}$ 
the end points of the arcs in $\Omega^\prime$ and let $r>0$ be such that 
$B_{4r}(x_i)\subseteq\Omega^\prime$ for all $i$, and 
$B_{4r}(x_i)\cap B_{4r}(x_j)=\emptyset$ if $i\neq j$.
Theorem~\ref{t:eps_salto_puro} yields 
that $\nabla u$ has a $C^{0,\alpha}$ extension on both sides of 
$(\Omega^{\prime\prime}\cap K)\setminus\cup_i\overline{B_{r}(x_i)}$
for all $\alpha<1$. In particular, $\nabla u$ is bounded on 
$\overline{\Omega^\prime}\setminus\cup_iB_{2r}(x_i)$.

Next consider the sequence $r_k=\frac r{2^{k-1}}$, $k\geq 0$, and fix 
$i\in\{1,\ldots,N\}$. Then, by Theorem~\ref{t:minimizers compactness} 
we can extract a subsequence $k_j\uparrow\infty$ along which the blow-up 
sequence $u_{x_i,r_{k_j}}(y):=r_{k_j}^{-1/2}u(x_i+r_{k_j}y)$ converge to 
some generalized (global) minimizer $(K,v,\{p_{kl}\})$.

By Proposition~\ref{p:monotonia-0} only two possibilities 
occur: either $x_i$ is a triple junction point, i.e., $K$ is a triple 
junction and $w$ is locally constant on $B_4\setminus K$, or $x_i$ is 
a cracktip (note that in this argument we do not need to know that 
the blow-up limit is unique).

In both cases, we claim that $\nabla u_j$ has a $C^{0,\alpha}$ 
extension on the closure of each connected component of 
$U_j:=(B_3\setminus\overline{B_1})\setminus K_{x_j,r_j}$ with 
$\sup_j\|\nabla u_{j}\|_{L^\infty(U_j)}\le C$. This follows as in 
\cite[Theorem 7.49]{AFP00} locally straightening 
$K_{x_j,r_j}\cap(B_4\setminus\overline{B_{1/2}})$ onto 
$K\cap(B_4\setminus\overline{B_{1/2}})$ via a $C^{1,\alpha}$ 
conformal map, a reflection argument and standard Schauder 
estimates for the laplacian.
Scaling back the previous estimate gives 
\[
|\nabla u(x)|\leq C\,|x-x_i|^{-1/2}\quad\text{ for } x\in
\cup_{j\in\N}(\overline{B_{3r_{k_j}}(x_i)}\setminus B_{r_{k_j}}(x_i)),
\] 
in turn from this, the maximum principle and Hopf's lemma we infer 
\[
|\nabla u(x)|\leq C\,r_k^{-1/2}\quad\text{ for } x\in 
B_{2r}(x_i)\setminus B_{r_k}(x_i).
\]
The latter inequality finally implies $\nabla u\in L^{4,\infty}(B_{2r}(x_i))$. 

Eventually, we are able to conclude $\nabla u\in L^{4,\infty}(\Omega^\prime)$, 
being on one hand $\nabla u$ bounded on 
$\overline{\Omega^\prime}\setminus\cup_iB_{2r}(x_i)$, and on the other hand 
belonging to $L^{4,\infty}(\cup_iB_{2r}(x_i))$.
\end{proof}

\subsection{Hausdorff dimension of the set of triple-junctions }\label{ss:cpt}

In order to prove Theorem~\ref{t:AFH2} we need to analyze the asymptotic behavior of minimizers of the Mumford and Shah energy in points where the scaled Dirichlet energy
is vanishing.
The approach developed by Ambrosio, Fusco and Hutchinson rests upon the notion of \emph{Almgren's area minimizing sets}, i.e.~a 
$\HH^1$ rectifiable set $S\subset B_1$ such that 
\[
\HH^1(S)\leq\HH^1(\varphi(S)),\quad
\forall\varphi\in\mathrm{Lip}(\R^2,\R^2),\,\,
\{\varphi\neq\mathrm{Id}\}\subset\hskip-0.125cm\subset B_1
\]
(cf.  \cite[Proposition 5.3, Theorem 5.4]{AFH}).
Theorem~\ref{t:AFH2} is then a consequence of a delicate study of the behavior of the composition of $SBV$ functions with Lipschitz deformations that are not necessarily one-to-one, and some specifications on the regularity theory for Almgren's area minimizing sets 
are needed (cf. \cite{AFH}). Hence, Theorem~\ref{t:AFH1} 
is a straightforward corollary of a much deeper and technically demanding result (given the higher integrability for granted). 

More recently, a different approach developed in the framework of Caccioppoli partitions, naturally related to the $SBV$ theory, has been developed in \cite[Proposition~5.1]{DLF13}. More generally, as shown in \cite{DLF13}, Caccioppoli partitions arise as limits of sequences of minimizers with vanishing $L^1$ gradient norms.\footnote{We point out that the results in \cite{AFH} and \cite{DLF13} have a higher dimensional counterpart.}

In Theorem~\ref{t:rH} below we give yet another proof  based on the characterization of elementary global minimizers stated in Theorem \ref{t:class-global}.
Let us first recall a technical lemma (see for instance
Section~3.6 \cite{Simon83} and 
\cite[Theorem~2.56, formula (2.43)]{AFP00}).
\begin{lemma}\label{l:haus}
 Let $s\geq 0$, then
 \begin{itemize}
  \item[(i)] $\HH^s(U)=0\Longleftrightarrow\HH^{s,\infty}(E)=0$, for all sets $U\subseteq\R^n$;
  \item[(ii)] if $U_j$ and $U$ are compact sets such that 
  $\sup_{U_j}\mathrm{dist}(\cdot,U)\downarrow 0$ as $j\uparrow\infty$, then
\[
\HH^{s,\infty}(U)\geq \limsup_j\HH^{s,\infty}(U_j);
\]
  \item[(iii)] if $\HH^s(U)>0$, then for $\HH^s$-a.e. $x\in U$
  \[
  \limsup_{\rho\downarrow 0^+}\frac{\HH^{s,\infty}(U\cap B_\rho(x))}{\omega_s\rho^s}\geq 2^{-s}\,.
  \]
 \end{itemize}
\end{lemma}
The strategy of proof below is essentially that by Ambrosio, Fusco and Hutchinson (see also \cite{DFR14}).
\begin{proof}[Proof of Theorem~\ref{t:AFH2}]
We argue by contradiction: suppose that 
$\HH^s(\Sigma^{(1)})>0$ for some $s\in(0,1)$,
%Therefore, $\HH^{s,\infty}(\Sigma^{(1)})>0$, and 
then for $\HH^s$-a.e. $x\in \Sigma^{(1)}$ 
\begin{equation}\label{e:limsup}
\limsup_{\rho\to 0}
\frac{\HH^{s,\infty}(\Sigma^{(1)}\cap B_\rho(x))}{\rho^s}
\ge \frac{\omega_s}{2^s}.
\end{equation}
Without loss of generality, assume that \eqref{e:limsup} holds at $x=0$, and 
consider a sequence $r_j\downarrow 0$ for which
\begin{equation}\label{e:assurdo}
\HH^{s,\infty}(\Sigma^{(1)}\cap B_{r_j})\ge\frac{\omega_s}{2^{s+1}}r_j^s
\qquad\text{for all $k\in\N$}.
\end{equation}
We blow-up $(K,u)$ at $0$ using the sequence $r_j$. Theorem~\ref{t:minimizers compactness} provides a subsequence, not relabeled for convenience, and an elementary global minimizer $(K_\infty,u_\infty)$ of $E_0$ such that for all open sets $A\subseteq B_1$
\begin{equation}\label{e:narrow}
\lim_j\HH^1(K_j\cap A)=\HH^1(K_\infty\cap A)\,,
\end{equation}
and that locally Hausdorff in $B_1$
\begin{equation}\label{e:DeLF}
K_j\to K_\infty\,.
\end{equation}

We claim that for every open cover $\mathcal{F}=\{F\}$ of $\Sigma_\infty\cap \overline B_1$, then   
\begin{equation}\label{e:usc}
r_j^{-1}\Sigma^{(1)}\cap\overline B_1\subseteq 
\cup_{F\in\mathcal{F}}F\,
\end{equation}
for every $j\ge j_0$, for some $j_0\in\N$. 
Indeed, if this were not the case we could find a sequence 
$x_k\in r_{j_k}^{-1}\Sigma^{(1)}\cap\overline B_1$ 
converging to some point $x_\infty$ not belonging to  $\Sigma_\infty$, the singular set of $K_\infty$. 
Thus, if $x_\infty+\mathcal{V}_\infty$ is the tangent plane to $K_\infty$ at $x_\infty$
(which exists by the very definition of $\Sigma_\infty$), then for some $\rho_0$ we would have
for every $\rho\in(0,\rho_0)$ {\color{red}{qui o dopo serve l'equivalenza tra $\beta$ e la piattezza media che segue dalla regolarità Ahlfors di $K$}}
\[
\rho^{-2}
\mathrm{dist}^2_H(K_\infty\cap B_{2\rho}(x_\infty),
(x_\infty+\mathcal{V}_\infty)\cap B_{2\rho}(x_\infty))<\varepsilon_0\,.
\]
The convergence in \eqref{e:narrow} would then imply 
for every $\rho\in(0,\rho_0\wedge 1)$
\[
\limsup_{k\uparrow\infty}\rho^{-2}\mathrm{dist}^2_H
(K_{j_k}\cap B_{2\rho}(x_k),(x_\infty+\mathcal{V}_\infty)\cap B_{2\rho}(x_\infty))<\varepsilon_0.
\]
In conclusion, being $x_k\in r_{j_k}^{-1}\Sigma^{(1)}$, we would get for $k$ large enough and for some $\theta_\infty\in[0,2\pi]$
\[
\limsup_{\rho\to 0}
\Omega^j(\theta_\infty,x_k,\rho)<\varepsilon_0,
\]
a contradiction to the definition of singular set. 

Hence, by \eqref{e:usc} we infer that
\[
\HH^{s,\infty}(\Sigma_\infty\cap\overline{B_1})\geq
\limsup_{j\uparrow\infty}\HH^{s,\infty}(r_j^{-1}\Sigma^{(1)}\cap\overline{B_1})\,.
\]
Given this, \eqref{e:assurdo} and \eqref{e:DeLF} yield that
\[
\HH^s(\Sigma_\infty\cap \overline{B_1})\ge\HH^{s,\infty}(\Sigma_\infty\cap\overline{B_1})\ge
\limsup_{k\uparrow\infty}\HH^{s,\infty}(r_j^{-1}\Sigma^{(1)}\cap\overline{B_1})\ge
\frac{\omega_s}{2^{s+1}},
\]
thus contradicting the density upper bound 
\eqref{e:upper bound}.
\end{proof}
\begin{corollary}\label{c:tj}
Let $(K,u)$ be a restricted, absolute, or generalized global minimizer of $E_\param$ in $\Omega\subseteq\R^2$, then $\Sigma^{(1)}$ is at most countable.
\end{corollary}
\begin{proof}
This claim follows straightforwardly from the compactness result Theorem~\ref{t:minimizers compactness}, 
the $\varepsilon$-regularity theory in Theorem~\ref{t:eps_tripunto}, and 
a direct application of Moore's triod theorem showing that in the plane 
every system of disjoint triods, i.e.~unions of three Jordan arcs that 
have all one endpoint in common and otherwise disjoint, is at most countable
(see \cite[Theorem~1]{Moore} and \cite[Proposition~2.18]{Pommerenke}). 
\end{proof}

We conclude the section by justifying  in $2$d the denomination used for the sets $\Sigma^{(1)}$ and 
$\Sigma^{(2)}$.
\begin{proposition}\label{p:bupchar}
Let $(K,u)$ be a restricted, absolute, or generalized global minimizer of $E_\param$ in $\Omega\subseteq\R^2$, then
 \begin{itemize}
  \item[(i)] $x\in\Sigma^{(1)}$ if and only if every blow-up of $(K,u)$ at $x$ is a global triple junction;
  \item[(ii)] $x\in\Sigma^{(2)}$ if and only if  every blow-up of $(K,u)$ at $x$ is a global cracktip.
  \end{itemize}
\end{proposition}
\begin{proof}
Given an infinitesimal sequence $r_j$ we use Theorem \ref{t:minimizers compactness} to blow-up $(K,u)$ at $x$, and denote by $(K_\infty,u_\infty)$ one such limit.
Recall that $(K_\infty,u_\infty)$ is a global minimizer of $E_0$. 

We begin with the direct implications of the statements above. In case (i), Theorem~\ref{t:class-global} yields that $(K_\infty,u_\infty)$ is an elementary global minimizers in turn implying straightforwardly that it is actually a global triple junction being $x\in\Sigma^{(1)}$. {\color{red}{anche qui si usa l'equivalenza fra $\beta$ e la piattezza media}}


Instead, in case (ii), being $x\in\Sigma^{(2)}$ for 
$\mathcal{L}^1$ a.e. $\rho>0$
\begin{align*}
\lim_{j}\beta(x,\rho\,r_j)&=
\lim_{j}\min_{\VV \in \mathcal{A}}\int_{B_\rho(x) \cap K_{x,r_j}} \frac{\dist^2(y,\VV)}{\rho^2} \, \frac{d \mathcal{H}^1(y)}{\rho}\\
&=\min_{\VV \in \mathcal{A}}\int_{B_\rho(x) \cap K_\infty} \frac{\dist^2(y,\VV)}{\rho^2} \, \frac{d \mathcal{H}^1(y)}{\rho}=0\,.
\end{align*}
Thus, $K_\infty$ is contained in a $1$-dimensional 
vector space. 
Then, a result by L\'eger \cite{Leger} ensures 
that $K_\infty$ is either empty or a line or a half line (cf. \cite[Theorem~64.1]{DavidBook}).
On the other hand, the energy upper bound in \eqref{e:upper bound} and being $x\in\Sigma^{(2)}$ yield for $ \mathcal{L}^1$ a.e. $\rho>0$
\begin{equation}\label{e:dircontra}
\lim_{j}d(x,\rho\,r_j)=\lim_{j}
\int_{B_\rho}|\nabla u_{x,r_j}|^2=
\int_{B_\rho}|\nabla u_\infty|^2
\in[\e_0,2\pi\,\rho].
\end{equation}
We claim that $K_\infty\neq\emptyset$. Otherwise, $|\nabla u_\infty|^2$ would be subharmonic on $\R^2$, being $u_\infty$ harmonic there, and thus we would deduce that
\[
 \sup_{B_{\frac r2}}|\nabla u_\infty|^2\leq \frac{4}{\pi r^2}\int_{B_r}|\nabla u_\infty|^2
 \stackrel{\eqref{e:upper bound}}{\leq}\frac 8r.
\]
As $r\uparrow\infty$ we would conclude that $u_\infty$ is constant, in contrast to \eqref{e:dircontra}. 

We claim that $K_\infty$ is not a line. Otherwise, $u_\infty$ would be harmonic in $\R^2\setminus K_\infty$.
Considering the restriction of $u_\infty$ to one of the two half-spaces forming $\R^2\setminus K_\infty$ and 
performing an even reflection, since $u_\infty$ satisfies a Neumann condition on $K_\infty$ we would get 
an harmonic function $w$ on $\R^2$ satisfying for all $r>0$
\[
 \int_{B_r}|\nabla w|^2\leq 4\pi r.
\]
Arguing as before $w$ would be constant. Hence, $u_\infty$ would be locally constant on 
$\R^2\setminus K_\infty$, leading again to a contradiction to \eqref{e:dircontra}. 

Therefore, $K_\infty$ is a half-line. Up to a rotation assume that 
$K_\infty=\{(x,0):\,x\leq 0\}$. Then the map $w:\{z\in\mathbb{C}:\,\mathrm{Re}z\geq 0\}\to\R$
defined by $w(z):=u_\infty(z^2)$ is harmonic and satisfying Neumann conditions on $\{\mathrm{Re}z= 0\}$ and additionally
\begin{equation}\label{e:tildew}
 \int_0^r\int_{-\sfrac\pi 2}^{\sfrac\pi 2}\Big(\rho\Big|\frac{\partial w}{\partial r}\Big|^2
 +\frac1\rho\Big|\frac{\partial w}{\partial \theta}\Big|^2\Big)d\rho\, d\theta
=\int_{B_{r^2}}|\nabla u_\infty|^2\leq 2\pi r^2.
\end{equation}
In view of \eqref{e:tildew}, the even extension of $w$ on $B_1$, 
that we still denote by $w$, has Fourier decomposition
\[
 w(r,\theta)=\alpha_0+\beta_1\,r\,\sin\theta.
%\sum_{k\geq 0}\rho^k\Big(\alpha_k\cos(k\theta)+\beta_k\sin(k\theta)\Big)
\]
Changing back coordinates and taking into account the minimality of $u_\infty$ (cf. Proposition \ref{p:constant-crack-tip}) we get
 \[
 u_\infty(r\cos\theta,r\sin\theta)=\alpha_0\pm\sqrt{\frac 2\pi r}\,\sin\frac\theta 2,
\]
the conclusion follows at once.

The reverse implications in both cases are easily concluded. Indeed, in case (i) let
 $(r_j)_j$ be satisfying
\[
\lim_jd(x,r_j)=\limsup_{r\downarrow 0} d(x,r)\,.
\]
Thus, any cluster point $(K_\infty,u_\infty)$ of 
$(K_{x,r_j},u_{x,r_j})$ is a triple junction function by 
assumption. Theorem \ref{t:minimizers compactness} then 
yields that for $\mathcal{L}^1$ a.e. $r>0$
\[
 \lim_j d(x,r_j)=\int_{B_r}|\nabla u_\infty|^2=0,
\]
so that $x\in \Sigma^{(1)}$.

Similarly, the reverse implication in case (ii) can be proved.
\end{proof}

Actually, in the first instance of Proposition~\ref{p:bupchar} uniqueness of the 
blow-up limit is ensured by Theorem~\ref{t:eps_tripunto}. As already remarked, 
case (ii) is still open in general.



\subsection{Higher integrability of the gradient via a reverse H\"older inequality}\label{ss:reverse holder}

Following a classical path, the key ingredient used in \cite[Theorem 1.3]{DLF13} 
to establish Theorem~\ref{t:hi} (for $E_0$) is a reverse H\"older inequality for the gradient, which we state independently. 
\begin{theorem}\label{t:rH}
For all %$\Lambda>0$ and 
$q\in(1,2)$ there exist $C_0>0$, $r_0\in(0,1)$ such that if $(K,u)$ is either a restricted, or an absolute, or a generalized global minimizer of $E_\param(\cdot,\cdot,B_1,g)$, with $\lambda\leq 1$, $\|g\|_{L^\infty}\leq M_0$ (we use the notation introduced in  Assumption~\ref{a:blow-up}), then for every $x\in B_{\sfrac12}$ and $r\in(0,r_0)$
\begin{equation}\label{e:rH}
\left(\fint_{B_r(x)\setminus K}|\nabla u|^2\right)^{\sfrac 12}
\leq C_0\left(\fint_{B_{2r}(x)\setminus K}|\nabla u|^q
\right)^{\sfrac1q}+C_0\|g\|_{L^\infty}\,.
\end{equation}
\end{theorem}
Theorem~\ref{t:hi} is then a consequence of a by now classical result 
by Giaquinta and Modica \cite{GM}. 
\begin{theorem}
Let $v\in L^q_{loc}(\Omega)$, $q>1$, be nonnegative such that for some
constants $\beta>0$, $t\geq 1$ and $R_0>0$
 \[
  \left(\fint_{B_r(z)}v^q\right)^{\sfrac 1q}\leq 
  \beta\fint_{B_{t\,r}(z)}v+\fint_{B_{t\,r}(z)}h
 \]
for all $z\in\Omega$, $r\in\left(0,R_0\wedge \mathrm{dist}(z,\partial\Omega)\right)$, 
and with $h\in L^s(\Omega)$ for some $s>1$.

Then $v\in L^p_{loc}(\Omega)$ for some $p>q$ and there is $C=C(\beta,n,q,p,\lambda)>0$
 such that 
 \[
 \left(\fint_{B_r(z)}v^p\right)^{\sfrac 1p}\leq C\,
 \left(\fint_{B_{2r}(z)}v^q\right)^{\sfrac 1q}
   +C\left(\fint_{B_{2r}(z)}h^q\right)^{\sfrac 1q}.
 \]
\end{theorem}
We provide here a new proof of Theorem~\ref{t:rH} relying on 
the compactness properties established in Theorem~\ref{t:minimizers compactness} rather than on the theory of Caccioppoli partitions as originally done in \cite{DLF13}. Nevertheless, the overall strategy is the same. 
\begin{proof}[Proof of Theorem~\ref{t:rH}]
Assume by contradiction that there is $q\in(1,2)$ such that for every $j\in\N$ one can find $(K_j,u_j)$ either restricted, or absolute, or generalized global minimizer of $E_{\param_j}(\cdot,\cdot,B_1,g_j)$ with ${\param_j}\leq 1$ and $\|g_j\|_{L^\infty}\leq M_0$, radii $r_j\downarrow 0$, and 
points $x_j\in B_{\sfrac12}$ such that
\begin{equation}\label{e:hpcontrad}
j\left(\fint_{B_{2r_j}(x_j)\setminus K_j}
|\nabla u_j|^q\right)^{\sfrac1q}+j\|g_j\|_{L^\infty}\leq
\left(\fint_{B_{r_j}(x_j)\setminus K_j}|\nabla u_j|^2\right)^{\sfrac 12}
\end{equation}
Consider the rescalings $(\widetilde{K}_j,\widetilde{u}_j):=((K_j)_{x_j,r_j}, (u_j)_{x_j,r_j})$, the conditions 
in Assumption~\ref{a:blow-up} are satisfied, then by Theorem~\ref{t:minimizers compactness} $(\widetilde{K}_j,\widetilde{u}_j)$ converge up to a subsequence to 
a blow-up limit $(K_\infty,u_\infty)$ which is a global generalized (restricted) minimizer of $E_0$ (in case $(K_j,u_j)$ are restricted minimizers). 
Moreover, by \eqref{e:hpcontrad} and the density upper bound \eqref{e:upper bound} 
we get
\[
\left(\fint_{B_2\setminus \widetilde{K}_j}|\nabla \widetilde{u}_j,|^q\right)^{\sfrac1q}\leq j^{-1}
\left(\fint_{B_1\setminus \widetilde{K}_j}|\nabla \widetilde{u}_j|^2\right)^{\sfrac 12}
\leq j^{-1}(2\pi+\lambda_j\pi M_0^2r_j)^{\sfrac 12}\,.
\]
The latter inequality and Theorem~\ref{t:minimizers compactness} 
yield that
\[
\lim_j\int_{B_2\setminus \widetilde{K}_j}|\nabla \widetilde{u}_j|^2=
\int_{B_2\setminus K_\infty}|\nabla u_\infty|^2=0.
\]
Therefore, Corollary~\ref{c:no-vanishing} implies that $(K_\infty,u_\infty)$ is an elementary global minimizer; in turn, this and Theorem~\ref{t:minimizers compactness} imply that for every $R>0$
\begin{equation}\label{e:enrg conv to glob min}
    \lim_j\int_{B_R\setminus \widetilde{K}_j}|\nabla \widetilde{u}_j|^2=0\,.
\end{equation}
In particular, $(K,u)$ is either a constant, or a global pure jump or a global triple junction (cf. Theorem \ref{t:class-global}). In any case, for all $R>0$
\begin{equation*}\label{e:enrg conv to glob min 2}
\mathcal{H}^0(K_\infty\cap\partial B_R)\leq 3,\qquad
\mathcal{H}^1(K_\infty\cap B_R)\leq 3R\,.
\end{equation*}
With fixed $R>0$ we shall now choose a radius $\rho\in[\frac R4,R]$ conveniently as outlined in what follows
\begin{itemize}
    \item[(a$_1$)] if $\mathcal{H}^0(K_\infty\cap\partial B_R)=0$ choose $\rho=R$; 
    \item[(a$_2$)] if $\mathcal{H}^0(K_\infty\cap\partial B_R)=2$ then $K_\infty\cap B_R$ is a segment and $\partial B_R\setminus K_\infty$ is the union two arcs. Then, either each of them has length less or equal to $\frac{4\pi}3R$ or $K\cap B_{\frac R2}=\emptyset$. In the first instance set $\rho=R$, in the second $\rho=\frac R2$;
    \item[(a$_3$)] if $\mathcal{H}^0(K_\infty\cap\partial B_R)=3$, then $K_\infty\cap B_R$ is a (possibly off-centered) propeller and $\partial B_R\setminus K_\infty$ is the union three arcs. 
    Then, either each of them has length less or equal to $(2\pi-\frac18)R$, in this case set $\rho=R$, or $\mathcal{H}^0(K_\infty\cap\partial B_{\frac R2})=2$.
    In the last event we are back to the setting of item (a2) with the radius $\frac R2$ playing the role of $R$. Thus, $K_\infty\cap B_{\frac R2}$ is a segment and $\partial B_{\frac R2}\setminus K_\infty$ is the union two arcs, and either each of them has length less or equal to $\frac{2\pi}3R$ or $K\cap B_{\frac R4}=\emptyset$. In the first instance set $\rho=\frac R2$, in the second $\rho=\frac R4$.
\end{itemize}
By \eqref{e:enrg conv to glob min} and Theorem~\ref{t:minimizers compactness} we may select $j_0\in\N$ such that for all $j\geq j_0$
\[
\int_{B_\rho\setminus \widetilde{K}_j}|\nabla \widetilde{u}_j|^2+\dist^2_H(\widetilde{K}_j\cap B_\rho),K_\infty\cap B_\rho)\leq\e \rho\,.
\]
Therefore, thanks to Theorem \ref{t:eps_salto_puro} and
Theorem \ref{t:eps_tripunto} for all $j\geq j_0$ and for some $\beta\in(0,\frac13)$ one of the following alternatives is true
\begin{itemize}
    \item[(b$_1$)] $\widetilde{K}_j\cap B_\rho=\emptyset$;
    \item[(b$_2$)] For each $t\in ((1-\beta)\rho,\rho)$,  
  $\partial B_{t}\setminus \widetilde{K}_j$ is the union of two arcs 
  $\gamma_1^j$ and $\gamma_2^j$ each with length $< (2\pi-\frac{1}{9})t$, 
  whereas $\widetilde{K}_j\cap B_t$ is connected and divides $B_t$ in two components 
  $B_1^j$, $B_2^j$ with $\partial B_i^j=\gamma_i^j\cup 
  (\widetilde{K}_j\cap\overline{B_t})$;

  \item[(b$_3$)] For each $t\in ((1-\beta)\rho, \rho)$, $\partial B_{t}\setminus \widetilde{K}_j$ 
is the union of three arcs 
  $\gamma_1^j$, $\gamma_2^j$ and $\gamma_3^j$ each with length $<(2\pi-\frac{1}{9})t$, whereas
  $B_t\cap \widetilde{K}_j$ is connected and divides $B_t$ in three connected 
  components $B_1^j$, $B_2^j$ and $B_3^j$ with 
  $\partial B_i^j\subset\gamma_i^j\cup  (\widetilde{K}_j\cap \overline{B_t})$.
\end{itemize}
We finally choose $r\in((1-\beta)\rho,\rho)$ and a subsequence, not relabeled, such that
\begin{itemize}
 \item[(A)] $h_j:=\widetilde{u}_j|_{\partial B_r}$ belongs to $W^{1,2}(\gamma)$ 
 for any connected component $\gamma$ of $\partial B_r\setminus \widetilde{K}_j$;

 \item[(B)] $h_j$ satisfies 
 \[
\int_{\partial B_r\setminus \widetilde{K}_j}
|h_j^\prime|^q d\HH^1
\leq\frac 1{\beta \rho}\int_{B_{\rho}}|\nabla \widetilde{u}_j|^q\,.
 \]
\end{itemize}
Let us conclude our argument by showing that \eqref{e:hpcontrad} is 
violated for $j$ sufficiently big. To this aim we note first that 
the choices $\beta<\frac13$ yields that $r>\frac23\rho$.

In case (b$_1$) holds, $\partial B_r\cap \widetilde{K}_j=\emptyset$ and $\widetilde{u}_j$ 
is the harmonic extension of its boundary trace $h_j$. Hence, the embedding $W^{1,q}(\partial B_r)\to H^{\sfrac12}(\partial B_r)$ implies for some constant $C>0$ (independent of $j$)
\begin{align*}
\int_{B_{\frac23\rho}} |\nabla \widetilde{u}_j|^2& \leq \int_{B_r}|\nabla \widetilde{u}_j|^2
\leq C\min_c \|h_j-c\|_{H^{\sfrac12}(\partial B_r)}^2\\ 
&\leq C\,\left(\int_{\partial B_r}|h_j^\prime|^q\,d\HH^1\right)^{\sfrac2q}
\stackrel{(B)}{\leq} C\,
\left(\frac 1{\beta \rho}\int_{B_\rho}
|\nabla \widetilde{u}_j|^q\right)^{\sfrac2q}\,.
\end{align*}
Choosing $R\geq 6$ and scaling back, we get a contradiction to \eqref{e:hpcontrad}
as $\rho\in[\frac R4,R]$.

In case (b$_2$) or (b$_3$) hold the construction is similar.
Denote by $J_j$ a \emph{minimal connection} 
\index{minimal connection@ minimal connection} relative to $\widetilde{K}_j\cap\partial B_r$, i.e. a closed and connected set in $\overline{B}_r$ containing 
$\widetilde{K}_j\cap\partial B_r$ with shortest length.
Then $J_j$ splits $\overline{B_r}$ into two (case (b$_2$)) or three (case (b$_3$)) regions denoted by $B^i_r$.
Let $\gamma^i$ be the arc of $\partial B_r$ contained in the boundary of $B^i_r$. 
The ensuing Lemma~\ref{l:traceext} provides a function $w_j^i\in W^{1,2}(B_r)$ with boundary trace $h_j$ and satisfying for some absolute constant $C>0$
\begin{equation}\label{e:wij}
\int_{B_r}|\nabla w_j^i|^2\,\leq C
\left(\int_{\gamma^i}|h_j^\prime|^q\,d\HH^1\right)^{\sfrac2q}.
\end{equation}
Denote by $w_j$ the function equal to $w^i_j$ on $B^i_j$, equal to $\widetilde{u}_j$ on $B_{r_j^{-1}}(-x_j)\setminus \cup_i B^i_j$, and extend $J_j$ as 
$J_j\setminus B_r=\widetilde{K}_j\setminus B_r$. 
Clearly, $w_j\in H^1(B_{r_j^{-1}}(-x_j)\setminus J_j)$. 
Scaling back $(J_j,w_j)$ to $B_1$ we obtain a pair admissible to test the 
minimality of $(K_j,u_j)$. 
On setting $g_j:=r_j^{-\sfrac12}g(x_j+r_j \cdot)$, for some constant $C>0$ 
we then deduce that
\begin{align*}%\label{e:explicit}
\int_{B_{\frac23\rho}\setminus \widetilde{K}_j}& |\nabla \widetilde{u}_j|^2 
\leq \int_{B_r\setminus \widetilde{J}_j}|\nabla \widetilde{u}_j|^2\notag\\ 
&\leq\int_{B_r\setminus \widetilde{J}_j}|\nabla w_j|^2 +
\underbrace{\HH^1 (J_j\cap B_r) - \HH^1 (\widetilde{K}_j\cap B_r)}_{\leq 0}%\notag\\&
+\lambda\int_{B_r\setminus \widetilde{J}_j}|w_j-g_j|^2
-\lambda\int_{B_r\setminus \widetilde{K}_j}|\widetilde{u}_j-g_j|^2\\
&\leq\int_{B_r\setminus\widetilde{J}_j}|\nabla w_j|^2+C\|g_j\|_{L^\infty}^2\rho^2r_j%\notag\\&
\stackrel{(\ref{e:wij})}{\leq} C\left(\int_{\partial B_r\setminus \widetilde{K}_j}|h_j^\prime|^q\,d\HH^1\right)^{\sfrac2q}
+C\|g_j\|_{L^\infty}^2\rho^2\,r_j\notag\\
&\stackrel{(B)}{\leq} 
C\left(\frac 1{\beta \rho}\int_{B_\rho\setminus\widetilde{K}_j}|\nabla \widetilde{u}_j|^q\,\right)^{\sfrac2q}
+C\|g_j\|_{L^\infty}^2\rho^2r_j\,.
\end{align*}
By taking into account that $\rho\in[\frac R4,R]$, choosing $R\geq 6$ and scaling back 
we find a contradiction to \eqref{e:hpcontrad}.
\end{proof}
We finally prove an elementary extension result.
\begin{lemma}\label{l:traceext}
For any $q\in(1,2)$ there exists $C=C(q)> 0$ such that
the following holds. For any arc $\gamma\subseteq\partial B_1$ 
and any $h\in W^{1,q}(\gamma)$, there exists 
$w\in W^{1,2}(B_1)$ with trace $g$ on $\gamma$ and
\begin{equation}\label{e:extension}
\|\nabla u_\infty\|_{L^{2}(B_1)}\leq \frac{C}{(2\pi - \HH^1(\gamma))^{1-\frac{1}{q}}}\, 
\|h^\prime\|_{L^{q}(\gamma)}.
\end{equation}
In addition, if $h\in L^\infty(\gamma)$, then $\|w\|_{L^\infty(B_1)}\leq 2\|h\|_{L^\infty(\gamma)}$.
\end{lemma}
\begin{proof}
Let $\alpha$, $\beta\in\partial B_1$ denote the extreme points of 
$\gamma$. By the H\"older inequality
\[
|h(\alpha)-h(\beta)|=\left|\int_\gamma h^\prime d\HH^1\right|
\leq(\HH^1(\gamma))^{1-\frac 1q}\|h^\prime\|_{L^q(\gamma)}\,.
\]
Linearly interpolating $h$ on $\partial B_1\setminus\gamma$, 
we get an extension $\widetilde{h}\in W^{1,q}(\partial B_1)$ of $h$ satisfying the estimate
\begin{equation}\label{e:una}
\|\widetilde{h}^\prime\|^q_{L^q(\partial B_1\setminus \gamma)}
=(2\pi - \HH^1(\gamma))^{1-q}|h(\alpha)-h(\beta)|^q
\leq\left(\frac{\HH^1(\gamma)}{2\pi - \HH^1(\gamma)}\right)^{q-1}
\|h^\prime\|^q_{L^q(\gamma)}\,.
\end{equation}
In turn, if we set $\hat{h}:=\widetilde{h}-\fint_{\partial B_1} \widetilde{h}$, the 
Poincar\'e inequality and (\ref{e:una}) yield
\begin{equation}\label{e:due}
\|\hat{h}\|^q_{L^q(\partial B_1)}\leq C\|\widetilde{h}^\prime\|^q_{L^q(\partial B_1)}
\leq C\left(\frac{2\pi}{2\pi - \HH^1(\gamma)}\right)^{q-1}
\|h^\prime\|^q_{L^q(\gamma)}\,.
\end{equation}
The embedding $W^{1,q}(\partial B_1)\to H^{1/2}(\partial B_1)$ 
provides us with a function $v\in W^{1,2}(B_1)$ with boundary trace $\hat{h}$ and
such that
\[
\|\nabla v\|_{L^2(B_1)}%\int_{B_1}|\nabla v|^2
\leq C\|\hat{h}\|_{H^{1/2}(\partial B_1)}\leq
C\|\hat{h}\|_{W^{1,q}(\partial B_1)}\stackrel{(\ref{e:due})}{\leq}
\frac{C}{\left(2\pi - \HH^1(\gamma)\right)^{1-\frac 1q}}\,
\|h^\prime\|_{L^q(\gamma)}.
\]
By the latter inequality the function 
$w:=v+\fint_{\partial B_1}\widetilde{h}$ fulfills the assertions of the Lemma. 
\end{proof}





\subsection{Higher integrability of the gradient via the porosity of the set $K$}\label{ss:porosity}

A central role in the approach by De Philippis and Figalli \cite{DePFig14} to establish 
the higher integrability of the gradient in any dimension is based on 
the ensuing improvement of Theorem~\ref{t:eps_salto_puro} due to David \cite{david1996}, and in higher dimension to Rigot \cite{Rig00}, and Maddalena and Solimini \cite{MadSol01}. Here, we provide a proof in the two dimensional setting using again Theorem \ref{t:minimizers compactness}.

\begin{theorem}\label{t:RMS}
There are constants $C_1,\,r_1,\,\e_1>0$ such that for every 
$\e\in(0,\e_1)$ there exists $t_\e\in(0,\frac 12)$ with the following property. If $(K,u)$ is either a restricted, or an absolute, or a generalized global minimizer of $E_\param(\cdot,\cdot,B_2,g)$, with $\lambda\leq 1$, $\|g\|_{L^\infty}\leq M_0$ (we use the notation introduced 
in  Assumption~\ref{a:blow-up}), then for every $x\in K\cap B_{\sfrac12}$ and for every $r\in(0,r_1)$ there exist $y\in K\cap B_r(x)$ and $\rho\in(t_\e r,r)$ such that $B_\rho(y)\subset B_r(x)$ and the assumptions of Theorem~\ref{t:eps_salto_puro} are satisfied in $B_\rho(y)$, namely for some $\theta\in[0,2\pi]$
\[
\Omega^j(\theta,y,\rho)+\lambda\|g\|_{L^\infty}^2 \rho^{\frac12}< \e_0
\]
($\e_0>0$ being the constant in Theorem~\ref{t:eps_salto_puro}).

In addition, it is true that
\begin{itemize}
 \item[(i)] $ K\cap B_\rho(y)$ is a $C^{1,\alpha}$ graph;
 \item[(ii)] 
\begin{equation}\label{e:neureg}
 \rho\|\nabla u\|^2_{L^\infty(B_\rho(y))}\leq C_1\, \e.
\end{equation} 
\end{itemize}
\end{theorem}
\begin{proof}
Assume by contradiction that %for every $j\in\N$ 
we can find sequences $\e_j\downarrow 0$, $r_j\downarrow 0$, $(K_j,u_j)$ of either restricted, or absolute, or generalized global minimizers of $E_{\param_j}(\cdot,\cdot,B_2,g_j)$, with $\param_j\leq 1$, $\|g_j\|_{L^\infty}\leq M_0$, %such that there are 
points $x_j\in K_j\cap B_{\sfrac12}$, and
%constants $C_j>0$, 
scalars $t_j\in(0,\frac12)$ such that for every 
$y\in K_j\cap B_{r_j}(x_j)$ and $\rho\in(t_jr_j,r_j)$ with $B_{\rho}(y)\subset B_{r_j}(x_j)$, then  
\begin{equation}\label{e:contra porosity}
%\Omega^j(\theta,y,\rho)
    \rho^{-2}\dist_H^2 (K_j \cap B_{2\rho}(y), \mathcal{R}_{\theta} (\ello))\cap B_{2\rho}(y)) + \rho^{-1} \int_{B_{2\rho}(y)\setminus K_j} |\nabla u_j |^2+\lambda_j\|g_j\|_{L^\infty}^2 \rho^{\frac12}\geq \e_0\,
\end{equation}
for every $\theta\in[0,2\pi]$ (we are using the notation introduced at the beginning of Section \ref{s:epsilon reg}).

Consider the rescalings $(\widetilde{K}_j,\widetilde{u}_j):=((K_j)_{x_j,r_j},(u_j)_{x_j,r_j})$, being the conditions 
in Assumption~\ref{a:blow-up} satisfied, by Theorem~\ref{t:minimizers compactness} $(\widetilde{K}_j,\widetilde{u}_j)$ converge up to a subsequence to 
a blow-up limit $(K_\infty,u_\infty)$ which is a global generalized (restricted) minimizer of $E_0$ (in case $(K_j,u_j)$ are restricted minimizers). 
Moreover, Corollary~\ref{c:a.e.regularity} yields that the subset of $K_\infty$ of pure jump points is relatively open and has full $\mathcal{H}^1$ measure. 
Let $z\in K_\infty$ be one such point, then necessarily 
Theorem \ref{t:eps_salto_puro} implies that %$\Omega^j(\theta_z,z,\rho)< \e_0$ 
\[
 t^{-2}\dist_H^2 (K_\infty \cap B_{2t}(z), \mathcal{R}_{\theta_z} (\ello))\cap B_{2t}(z)) + 
 t^{-1} \int_{B_{2t}(z)\setminus K_\infty} 
 |\nabla u_\infty|^2< \e_0
 \]
for some $\theta_z\in[0,2\pi]$ and for every $t>0$ sufficiently small. 
In turn, Theorem \ref{t:minimizers compactness} implies 
the existence of points $z_j\in K_j\cap B_{r_j}(x_j)$ such that
\begin{align*}
    (t r_j)^{-2}&\dist_H^2 (K_j \cap B_{2{t r_j}}(z_j), \mathcal{R}_{\theta_z} (\ello))\cap B_{2t r_j}(z_j)) \\ 
    &+ (t r_j)^{-1} 
    \int_{B_{2t r_j}(z_j)\setminus K_j} |\nabla u_j |^2+\lambda_j\|g_j\|_{L^\infty}^2 (t r_j)^{\frac12}< \e_0\,
\end{align*}
contradicting \eqref{e:contra porosity}.

Item (i) follows directly from Theorem \ref{t:eps_salto_puro}; instead estimate \eqref{e:neureg} is a consequence of item (i) and classical elliptic regularity results for the Neumann problem since $u$ satisfies \eqref{e:Euler curvature g} and \eqref{e:Euler Neumann g} (cf. \cite[Theorem 7.53]{AFP00}).

{\color{red}{Si usa due volte la regolarit\'a di $\nabla u$ fino a $K$}}
\end{proof}

Theorem~\ref{t:RMS} can be rephrased by asserting that the set $\Sigma$ is $(t_\e,1)$-\emph{porous} in $K$ (cf. \cite[...]{mattila}).
\index{porosity @porosity}
Hence, the estimates on the Minkowski dimension
\index{Minkowski dimension @Minkowski dimension}
(and thus on the Hausdorff dimension) of the singular set $\Sigma$ contained in the papers by David \cite{david1996}, Rigot \cite{Rig00} and Maddalena and Solimini \cite{MadSol01} is a consequence of 
Theorem~\ref{t:RMS}, a by now classical result by David and Semmes~\cite{DavSem97}, and of the Alfhors regularity of $K$ (cf. Lemma~\ref{l:upper-bound} and Theorem~\ref{t:dlb}), which we restate for convenience: if $(K,u)$ is either an absolute, or a restricted or a generalized minimizer of $E_\param$ on $B_2$ then
\begin{equation}\label{e:SuAR}
\epsilon\,r \leq \HH^1( K\cap B_r(x)) \leq \e_\param r
\end{equation}
for some constant $\epsilon>0$, for $\e_\param:=(2  + \lambda \|g\|_\infty^2 )\pi$, for every $x\in  K$, and for every $r\in(0,1\wedge \mathrm{dist}(x,\partial\Omega))$.

Instead, in Proposition~\ref{p:alfpor} below it will be obtained directly. The key technical results to prove higher integrability are contained in Proposition~\ref{p:alfpor} for which we need two preparatory lemmas. 
The first one is obtained via De Giorgi's slicing/averaging principle.
\begin{lemma}\label{l:technical}
 There are positive constants $M_1$, $C_1$ such that if $M\geq M_1$ for every $(K,u)$ (absolute, restricted, generalized, or generalized restricted) minimizer of $E_\param$ on $B_2$ we can find three decreasing sequences of radii such that 
 \begin{itemize}
  \item[(i)] $1\geq R_h> S_h> T_h> R_{h+1}$;
  \item[(ii)] $8M^{-(h+1)}\leq R_h-R_{h+1}\leq M^{-\frac{(h+1)}2}$, and $S_h-T_h=T_h-R_{h+1}=4M^{-(h+1)}$;
  \item[(iii)] $\HH^1( K\cap( \overline{B}_{S_h}\setminus \overline{B}_{R_{h+1}}))\leq C_1M^{-\frac{(h+1)}2}$;
  \item[(iv)] $R_\infty=S_\infty=T_\infty\geq 1/2$.
  \end{itemize}
\end{lemma}
\begin{proof}
Let $R_1=1$, given $R_h$ we construct $S_h$, $T_h$ and $R_{h+1}$ as follows.

Set $N_h:=\lfloor \frac{M^{\frac{h+1}2}}8\rfloor\in\N$ and fix $M_1\in\N$ such that 
$N_h\geq \lfloor \frac{M^{\frac{h+1}2}}{16}\rfloor$ for $M\geq M_1$. Here, 
$\lfloor t\rfloor$ denotes the integer part of $t\in\R$. 

The annulus $B_{R_h}\setminus  \overline{B}_{R_h-8M^{-\frac{h+1}2}}$ contains the $N_h$ disjoint sub annuli 
$ \overline{B}_{R_h-8(i-1)M^{-(h+1)}}\setminus  \overline{B}_{R_h-8iM^{-(h+1)}}$, $i\in\{1,\ldots,N_h\}$, of equal 
width $8\,M^{-(h+1)}$. By averaging we can find an index $i_h\in\{1,\ldots,N_h\}$ such that
\begin{multline*}
\HH^1\big(K\cap( \overline{B}_{R_h-8(i_h-1)M^{-\frac{h+1}2}}\setminus \overline{B}_{R_h-8i_h\,M^{-\frac{h+1}2}})\big)\\
\leq \frac 1{N_h}\,\HH^1\big(K\cap ( \overline{B}_{R_h}\setminus  \overline{B}_{R_h-8M^{-\frac{h+1}2}})\big)
\stackrel{\eqref{e:SuAR}}{\leq} 
\varepsilon^{-1}\,\frac{R_h}{N_h}\leq 8\varepsilon^{-1}\,M^{-\frac{h+1}2},
\end{multline*}
so that (iii) is established with $C_1:=8\varepsilon^{-1}$. Finally, set 
\[
 S_h:=R_h-8(i_h-1)M^{-(h+1)},\,\,R_{h+1}:=R_h-8i_h\,M^{-(h+1)},\,\,T_h:=\frac12(S_h+R_{h+1}),
\]
then items (i) and (ii) follow by the very definition, and item (iv) from (ii) if 
$M_1$ is sufficiently big.
\end{proof}
The second lemma has a geometric flavor.
\begin{lemma}\label{l:grafico}
Let $f:\R^{n-1}\to\R$ be Lipschitz with
\begin{equation}\label{e:lip}
f(0)=0,\quad\|\nabla f\|_{L^\infty}\leq\eta.
\end{equation}
If $G:=\mathrm{graph}(f)\cap B_{2}$ and $\eta\in(0,\sfrac{1}{15}]$, then 
for all $\delta\in(0,\sfrac12)$ and $x\in (\overline{B}_{1+\delta}\setminus B_{1})\cap G$
\[
\mathrm{dist}(x,(\overline{B}_{1+2\delta}\setminus B_{1+\delta})\cap G)\leq \frac 32 \delta.
\]
\end{lemma}
\begin{proof}
Clearly by \eqref{e:lip} we get
\[
 \|f\|_{W^{1,\infty}(B_2)}\leq 3\eta.
\]
Let $x=(y,f(y))\in (\overline{B}_{1+\delta}\setminus B_{1})\cap G$ and $\hat{x}:=(\lambda\,y,f(\lambda\,y))$,
with $\lambda$ to be chosen suitably. Note that as $|x|\geq 1$ we have
\begin{align*}
 |f(\lambda\,y)-\lambda\,f(y)|&\leq |f(\lambda\,y)-f(y)|+|\lambda-1|\,|f(y)|\\
 &\leq |\lambda-1|\,(\|\nabla f\|_{L^\infty}\,|y|+\|f\|_{L^\infty})\leq 3\eta|\lambda-1|\,|x|.
\end{align*}
Hence,
\[
 |\hat{x}-x|\leq |\hat{x}-\lambda\,x|+|\lambda-1||x| \leq(3\eta+1)|\lambda-1|\,|x|.
\]
It is easy to check that the choice $\lambda=1+\frac{5}{4}\delta|x|^{-1}$ gives the conclusion.
\end{proof}

Following De Philippis and Figalli \cite{DePFig14}, we prove next a version of 
the mentioned porosity result by David and Semmes~\cite{DavSem97} suitable for our purposes.
In what follows, $(E)_r$ denotes the open $r$-neighborhood of a given a set $E$, i.e. 
$(E)_r=\{x\in\R^2:\,\dist(x,E)< r\}$.
\begin{proposition}\label{p:alfpor}
Let $\epsilon,\,C_1,\,M_1$ be the constants in \eqref{e:SuAR} and Lemma \ref{l:technical}, 
respectively.

There exist constants $C_2,\, M_2>0$ and $\alpha,\beta\in(0,\sfrac 14)$, 
with $M_2\geq M_1$, such that for every $M\geq M_2$, for every $(K,u)$ (absolute, restricted, generalized, or generalized restricted) minimizer of $E_\param$ on $B_2$, 
we can find families $ \mathcal{F}_j$ of disjoint balls
 \[
  \mathcal{F}_j=\left\{B_{\alpha M^{-j}}(y_i):\,y_i\in  K,\,1\leq j\leq N_j\right\}
 \]
such that for all $h\in\N$ 
\begin{itemize}
 \item[(i)] if $B$, $B^\prime\in\cup_{j=1}^h \mathcal{F}_j$ are distinct balls, then 
 $(B)_{4M^{-(h+1)}}\cap(B^\prime)_{4M^{-(h+1)}}=\emptyset$;
 \item[(ii)] if $B_{\alpha M^{-j}}(y_i)\subset \mathcal{F}_j$, then 
 $ K\cap B_{2\alpha M^{-j}}(y_i)$ is a $C^{1,\gamma}$ graph, $\gamma\in(0,1)$, 
 containing $y_i$,
 \[
\inf_\theta\Omega^j(\theta,y_i,2\alpha M^{-j})
+\lambda\|g\|^2_\infty(\alpha M^{-j})^{\frac12} 
< \e_0\,,
 \]
\begin{equation}\label{e:gradbdd}
\|\nabla u\|_{L^\infty(B_{2\alpha M^{-j}}(y_i))}<M^{j+1}; \end{equation}
 \item[(iii)] let $\{R_h\}_{h\in\N}$, $\{S_h\}_{h\in\N}$, $\{T_h\}_{h\in\N}$ be the sequences of radii in 
 Lemma~\ref{l:technical}, and let
 \[
  K_h:=( K\cap\overline{B}_{S_h})\setminus\left(\cup_{j=1}^h\cup_{ \mathcal{F}_j}B\right),
 \]
 (by construction $K_{h+1}\subset K_h\setminus \cup_{ \mathcal{F}_{h+1}}B$), and 
 \[
 \widetilde{K}_h:= ( K\cap\overline{B}_{T_h})\setminus
\left(\cup_{j=1}^h\cup_{ \mathcal{F}_j}(B)_{2M^{-(h+1)}}\right)\subset K_h.
 \]
 Then, there exists a finite set of points $ \mathcal{C}_h:=\{x_i\}_{i\in I_h}\subset\widetilde{K}_h$ such that
 \begin{equation}\label{e:centres}
  |x_j-x_k|\geq 3M^{-(h+1)}\quad\forall j,k\in I_h,\,j\neq k;
 \end{equation}
 \begin{equation}\label{e:ingro}
  (K_h\cap  \overline{B}_{R_{h+1}})_{M^{-(h+1)}}\subset 
	\cup_{i\in I_h}B_{8M^{-(h+1)}}(x_i);
 \end{equation}
 \begin{equation}\label{e:stimaKh}
  \HH^1(K_h)\leq C_1\,h\,M^{-2h\beta};
%   \HH^1(K_{h+1})\leq(1-\eta)\HH^1(K_h)+C_1M^{-\frac{(h+1)}2};
 \end{equation}
 \begin{equation}\label{e:measureingro}
   \mathcal{L}^2\left((K_h\cap  \overline{B}_{R_{h+1}})_{M^{-(h+1)}}\right)\leq C_2\,h\,M^{-h(1+2\beta)-1}.
  %	C_2 M^{-(h+1)}\HH^1(K_h).
 \end{equation}
 
 \item[(iv)] $\Sigma\cap B_{\sfrac12}\subset K_h$ for all $h\in\N$ and 
 \begin{equation}\label{e:sigmaur}
  \mathcal{L}^2\left((\Sigma\cap B_{\sfrac12})_{r}\right)\leq C_2\,r^{1+\beta}\qquad\forall r\in(0,\sfrac 12].
 \end{equation}
In particular, 
$\dim_{\MM}(\Sigma\cap B_{\sfrac12})\leq 1-\beta$.
 \end{itemize}
\end{proposition}
\begin{proof}%[Proof of Proposition~\ref{p:alfpor}]
In what follows we shall repeatedly use Theorem~\ref{t:RMS} 
with $ \e\in(0,1)$ fixed and sufficiently small. 
We split the proof in several steps.
\smallskip

\noindent{\bf Step 1.} \emph{Inductive definition of the families $ \mathcal{F}_j$.}

%We prove the result by induction. 
For $h=1$ we define 
 \[
 \mathcal{F}_1:=\emptyset,\,\, K_1=K\cap \overline{B}_{S_1},\,\,\widetilde{K}_1=K\cap \overline{B}_{T_1}, 
\] 
and choose $ \mathcal{C}_1$ to be a maximal family of points at distance $3M^{-2}$ 
from each other. 
Of course, properties in items (i) and (ii) and in \eqref{e:centres} are satisfied. 
To check the others, one can argue as in the verification below.
 
 Suppose that we have built the families $\{ \mathcal{F}_j\}_{j=1}^h$ as in the statement, to construct $\mathcal{F}_{h+1}$ we argue as follows. 
 Let $\mathcal{C}_h=\{x_i\}_{i\in I_h}\subset\widetilde{K}_h$ be a maximal family of points satisfying \eqref{e:centres}, i.e.~$|x_i-x_k|\geq 3M^{-(h+1)}$ for all $j,\,k\in I_h$ 
 with $j\neq k$. Consider 
 \[
 \mathcal{G}_{h+1}:=\{B_{M^{-(h+1)}}(x_i)\}_{i\in I_h}.
 \]
For every ball $B_{M^{-(h+1)}}(x_i)\in \mathcal{G}_{h+1}$ we can find a sub-ball $B_{2\alpha\,M^{-(h+1)}}(y_i)\subset B_{M^{-(h+1)}}(x_i)$,
 $\alpha\in(0,\sfrac 14)$ for which the theses of Theorem~\ref{t:RMS} are satisfied. Then, define
 \[
  \mathcal{F}_{h+1}:=\{B_{\alpha\,M^{-(h+1)}}(y_i)\}_{i\in I_h}.
 \]
 By condition \eqref{e:centres}, the balls $B_{\frac32 M^{-(h+1)}}(x_i)$ are disjoint and
 do not intersect
 \[
  \cup_{j=1}^h\cup_{ \mathcal{F}_j}(B)_{\frac12M^{-(h+1)}}
 \]
 by the very definition of $\widetilde{K}_h$. Thus, item (i) and (ii) are satisfied
 for $M_2$ sufficiently large. 
  Hence, we can define $K_{h+1}$, $\widetilde{K}_{h+1}$ and $ \mathcal{C}_{h+1}$ as in the statement. 
  
  We verify next the rest of the conclusions.  
\smallskip

 \noindent{{\bf Step 2.}} \emph{Proof of \eqref{e:ingro}.}
%We omit the proof of \eqref{e:ingro} that exploits a technical lemma in which the specific regularity 
%properties of $K= K$ come into play.

Let $x\in (K_{h+1}\cap  \overline{B}_{R_{h+2}})_{M^{-(h+2)}}$ and let $z$ be a point of minimal distance from $K_{h+1}\cap  \overline{B}_{R_{h+2}}$. 
In case $z\in \widetilde{K}_{h+1}$, by maximality of $\mathcal{C}_{h+1}$ there is some point $x_i\in  \mathcal{C}_{h+1}$ such that 
$|z-x_i|< 3M^{-(h+2)}$ and thus we conclude $x\in B_{4M^{-(h+2)}}(x_i)$.
Instead, if $z\in(K_{h+1}\cap  \overline{B}_{R_{h+2}})\setminus\widetilde{K}_{h+1}$, the definitions of ${K_{h+1}}$ and $\widetilde{K}_{h+1}$ yield the existence of a ball $\widetilde{B}\in\cup_{j=1}^{h+1} \mathcal{F}_j$ 
for which $z\in (K\cap(\widetilde{B})_{2M^{-(h+2)}})\setminus \widetilde{B}$. 
Item (ii) and a scaled version of Lemma \ref{l:grafico} 
(applied with $\delta=2M^{-(h+2)}$, and radii $\rho$ (that of $\widetilde{B}$) and $\rho+2M^{-(h+2)}$ in place of $1$ and $1+\delta$) give a point $y$ satisfying
\[
y\in \left(K\cap(\widetilde{B})_{4M^{-(h+2)}}\right)\setminus (\widetilde{B})_{2M^{-(h+2)}},\quad
\text{and}\quad |z-y|\leq 3M^{-(h+2)}.
\]
Therefore, as $z\in \overline{B}_{R_{h+2}}$ and $T_{h+1}=R_{h+2}+4M^{-(h+2)}$ 
we get by property (i) and the definition of $\widetilde{K}_{h+1}$ 
\[
y\in \left(K\cap B_{T_{h+1}}\cap(\widetilde{B})_{3M^{-(h+2)}}\right)
\setminus (\widetilde{B})_{2M^{-(h+2)}}\subset \widetilde{K}_{h+1}.
\]
Finally, by maximality of $\mathcal{C}_{h+1}$ we may find $x_i\in \mathcal{C}_{h+1}$ 
such that $|y-x_i|< 3M^{-(h+2)}$. In conclusion, we have
\[
|x-x_i|\leq|x-z|+|z-y|+|y-x_i|\leq 7M^{-(h+2)},
\]
so that  \eqref{e:ingro} follows at once.
\smallskip

\noindent{{\bf Step 3.}} \emph{For every $h\in\N$ and for every $x_i\in  \mathcal{C}_{h}$
\begin{equation}\label{e:dlbKh}
 K_{h}\cap B_{M^{-(h+1)}}(x_i)=K\cap B_{M^{-(h+1)}}(x_i)\,.
\end{equation}}
Indeed, assume by contradiction that we can find $x_i\in  \mathcal{C}_{h}$ and $x\in (K\setminus K_{h})\cap B_{M^{-(h+1)}}(x_i)$. 
As $x_i\in\widetilde{K}_{h}$ then $x_i\in B_{T_{h}}$, in turn implying 
$x\in B_{S_{h}}$ since $S_h-T_h=4M^{-(h+1)}$.
Therefore $x\in(K\setminus K_{h})\cap \overline{B}_{S_{h}}$, and by definition of 
$K_{h}$ we can find a ball $B\in  \mathcal{F}_{j}$, $j\leq h$, such that $x\in B$. 
We conclude that
\[
\textrm{dist}(x_i,B)\leq|x-x_i|\leq M^{-(h+1)},
\] 
contradicting that $x_i\in\widetilde{K}_{h}$.
\smallskip

\noindent{{\bf Step 4.}} \emph{Proof of \eqref{e:stimaKh}.}

We get first a lower bound for $\mathcal{H}^0(I_h)$: use \eqref{e:ingro} and the density upper bound in \eqref{e:SuAR} to get
 \[
  \HH^1(K_h\cap  \overline{B}_{R_{h+1}})=
  \HH^1(K_h\cap  \overline{B}_{R_{h+1}}
  \cap\cup_{i\in I_h}B_{8M^{-(h+1)}}(x_i))
  \leq \e_\param 8M^{-(h+1)}\,\mathcal{H}^0(I_h)
 \]
where we recall that $\e_\param=(2+\lambda \|g\|_\infty^2)\pi$.
Equivalently, we have that 
 \begin{equation}\label{e:Ihbound}
 \mathcal{H}^0(I_h)M^{-(h+1)}\geq \frac1{8\e_\param} 
 \HH^1(K_h\cap  \overline{B}_{R_{h+1}}).
 \end{equation}
 Thus, we estimate as follows by taking into account that by item (i) the balls in the  family $\mathcal{F}_{h+1}$ are disjoint 
 \begin{align}\label{e:measure}
  \HH^1(K_{h+1})&\leq\HH^1\left(K_h\setminus\cup_{ \mathcal{F}_{h+1}}B\right)
  =\HH^1(K_h)-\sum_{ \mathcal{F}_{h+1}}\HH^1(K_h\cap B)\notag\\
 &\stackrel{\eqref{e:SuAR},\,\eqref{e:dlbKh}}{\leq}
	\HH^1(K_h)-\epsilon \alpha M^{-(h+1)}\mathcal{H}^0(I_h) 
  \stackrel{\eqref{e:Ihbound}}{\leq}\HH^1(K_h)-
  \frac\epsilon{8\e_\param}\alpha
  \HH^1(K_h\cap  \overline{B}_{R_{h+1}})\notag\\
  &=(1-\eta)\HH^1(K_h)+\eta\left(\HH^1(K_h)-\HH^1(K_h\cap  \overline{B}_{R_{h+1}})\right)\notag\\
  &\leq(1-\eta)\HH^1(K_h)+\eta\,\HH^1(K\cap(\overline{B}_{S_h} \setminus  \overline{B}_{R_{h+1}}))\leq(1-\eta)\HH^1(K_h)+C_1M^{-\frac{h+1}2},
 \end{align}
where we have set $\eta:=\frac\epsilon{8\e_\param}\alpha$, and we have used the very definition of $K_h$ in the last but one inequality, and item of (iii) Lemma~\ref{l:technical} in the last one.
By iteration of \eqref{e:measure}, we find 
\[
 \HH^1(K_h)\leq C_1\sum_{i=1}^h(1-\eta)^{h-i}M^{-\sfrac i2}
 \leq C_1\,h\,(\max\{1-\eta,M^{-\sfrac 12}\})^h.
\]
Choose $\beta\in(0,\sfrac 14)$ such that $(1-\eta)\leq M^{-2\beta}$, 
the previous estimate then yields \eqref{e:stimaKh}, 
\begin{equation*}%\label
 \HH^1(K_h)\leq C_1\,h\,\max\{M^{-2h\beta},M^{-\sfrac h2}\}=C_1\,h\,M^{-2h\beta}.
\end{equation*}


\smallskip
 
 
 
 \noindent{{\bf Step 5.}} \emph{Proof of \eqref{e:measureingro}.}

We use \eqref{e:ingro} to get
 \begin{align*}%\label{e:rozza}
   \mathcal{L}^2\left((K_{h+1}\cap  \overline{B}_{R_{h+2}})_{M^{-(h+2)}}\right)&\leq 
   \mathcal{L}^2\left(\cup_{i\in I_{h+1}}B_{8M^{-(h+2)}}(x_i)\right)\leq 
	64 M^{-2(h+2)}\mathcal{H}^0(I_{h+1})\notag\\
  &\stackrel{\eqref{e:SuAR},\, \eqref{e:dlbKh}}{\leq} 64\epsilon M^{-(h+2)}\sum_{i\in 
	I_{h+1}}\HH^1(K_{h+1}\cap B_{M^{-(h+2)}}(x_i))\notag\\
  &\leq 64\epsilon M^{-(h+2)}\HH^1(K_{h+1})
  \stackrel{\eqref{e:stimaKh}}{\leq} 64\epsilon C_1\,(h+1)\,M^{-2(h+1)\beta-(h+2)}.
  \end{align*}
where in the last but one inequality we have used that the balls $B_{M^{-(h+2)}}(x_i)$ 
are disjoint by construction.
\smallskip
 
 


\noindent{{\bf Step 6.}} \emph{Proof of \eqref{e:sigmaur}}
  
By construction we have that $\Sigma\cap B_{\sfrac 12}\subseteq K_h$. 
Therefore, %\eqref{e:stimaKh} and 
\eqref{e:measureingro} gives as $R_h\geq R_\infty\geq\sfrac 12$
\begin{equation*}
\mathcal{L}^2\left((\Sigma\cap B_{\sfrac12})_{M^{-(h+1)}}\right)\leq
\mathcal{L}^2\left((K_{h}\cap\overline{B}_{R_{h+1}})_{M^{-(h+1)}}\right)
\leq C_2\,h\,M^{-h(1+2\beta)-1}. 
\end{equation*}
Hence, if $r\in (M^{-(h+2)},M^{-(h+1)}]$ we get
\[
  \mathcal{L}^2\big((\Sigma\cap B_{\sfrac12})_{r}\big)\leq 
 C_2\,h\,M^{-h(1+2\beta)-1}\leq  C_2\,M^{-h(1+\beta)-1}\leq C_2\,r^{1+\beta}.\qedhere
\]
\end{proof}

We are now ready to establish the higher integrability of 
the gradient.
\begin{theorem}\label{t:hiDePF}

There is $p>2$ such that for all open sets $\Omega\subseteq\R^2$ and for all 
$(K,u)$ either a restricted, or an absolute, or a generalized global minimizer of $E_\param(\cdot,\cdot,\Omega,g)$ then $\nabla u\in L^p_{\mathrm{loc}}(\Omega\setminus K)$ .
\end{theorem}
\begin{proof} 
Clearly, it is sufficient for our purposes to prove a localized estimate. Hence,
for the sake of simplicity we suppose that $ \Omega=B_2$. 

We keep the notation of Proposition~\ref{p:alfpor} and furthermore denote for all $h\in\N$ 
 \begin{equation}\label{e:Ah}
  A_h:=\{x\in B_2\setminus K:\,|\nabla u(x)|^2>M^{h+1}\}\,.
 \end{equation}
We claim that 
\begin{equation}\label{e:claimAh}
A_{h+2}\cap B_{R_{h+2}}\subset (K_h\cap B_{R_{h+1}})_{M^{-(h+1)}}.
\end{equation}
Given this for granted we conclude as follows: we use \eqref{e:measureingro} to deduce that 
\begin{equation}\label{e:estmeas}
 \mathcal{L}^2(A_{h+2}\cap B_{R_{h+2}})\leq \mathcal{L}^2\left((K_h\cap B_{R_{h+1}})_{M^{-(h+1)}}\right)\leq
%\\\stackrel{\eqref{e:measureingro}}{\leq}
%C_2\,M^{-(h+1)}\HH^1(K_h)\stackrel{\eqref{e:stimaKh}}{\leq} C_1\,
C_2\,h\,M^{-h(1+2\beta)-1}.
\end{equation}
Therefore, recalling that $\frac 12\leq R_\infty\leq R_h$, in view of \eqref{e:estmeas} 
and Cavalieri's formula for $q>1$ we get that 
\begin{align*}
 \int_{B_{\frac12}}|\nabla u|^{2q}&=q\int_0^{\infty}t^{q-1}
  \mathcal{L}^2(\{x\in B_{\sfrac12}\setminus K:\,|\nabla u(x)|^2>t\})dt\\
&\leq q\sum_{h\geq 3}\int_{M^h}^{M^{h+1}}t^{q-1}
  \mathcal{L}^2(\{x\in B_{\sfrac12}\setminus K:\,|\nabla u(x)|^2>t\})dt+M^{3q} \mathcal{L}^2(B_{\sfrac12})\\
&\leq \sum_{h\geq 0}M^{(h+4)q} \mathcal{L}^2(A_{h+2}\cap B_{\frac 12})
+M^{3q} \mathcal{L}^2(B_{\frac12})\\
&\leq C_2\,\sum_{h\geq 0}h\,M^{(h+4)q-h(1+2\beta)-1}+M^{3q} \mathcal{L}^2(B_{\frac12}).
 \end{align*}
 The conclusion follows at once by taking $q\in(1,1+2\beta)$ and $p=2q$.
\smallskip

 To conclude we prove formula \eqref{e:claimAh} in two steps. 
 
 \noindent{{\bf Step 1.}} \emph{For every $M> 0$ large enough, for every $h\in\N$ and for every $R\in(0,1]$ we have that}
 \begin{equation}\label{e:prelimAh}
  A_h\cap B_{R-2M^{-h}}\subset(K\cap {B_R})_{M^{-h}}\,. 
 \end{equation}
Indeed, for $x\in A_h\cap B_{R-2M^{-h}}$ let  $z\in K$ be such that $\mathrm{dist}(x,K)=|x-z|$.
If $|x-z|>M^{-h}$ then $B_{M^{-h}}(x)\cap K=\emptyset$ so that $u$ 
solves \eqref{e:Euler harmonic g}, i.e. $\triangle u=\lambda(u-g)$, on $B_{M^{-h}}(x)$.
Therefore, being the right hand side of the PDE in $L^\infty$, by elliptic regularty Lipschitz bounds \cite[estimate (4.45)]{GT} and the density upper bound in \eqref{e:SuAR}, as $x\in A_h$ we infer that
\[
 M^{h+1}\leq|\nabla u(x)|^2\leq 
 %\fint_{B_{M^{-h}}(x)}|\nabla u|^2\leq 2\,M^h,
 C\,M^h
\]
with $C$ depending on $\|g\|_{L^\infty}$. The latter estimate is clearly impossible for $M$ large enough. 
Furthermore, as $x\in B_{R-2M^{-h}}$ and $|x-z|\leq M^{-h}$ we conclude that $z\in B_R$.
\smallskip

\noindent{{\bf Step 2.}} \emph{Proof of \eqref{e:claimAh}.}

Since $R_{h+1}-R_{h+2}\geq 8M^{-(h+2)}$ (cf. (i) Lemma~\ref{l:technical}), we apply Step~1 to $A_{h+2}$ 
and $R=R_{h+1}$ and then \eqref{e:prelimAh} implies that 
\[
A_{h+2}\cap B_{R_{h+2}}\subset\big(K\cap B_{R_{h+1}}\big)_{M^{-(h+1)}}.
\]
Let $x\in A_{h+2}\cap B_{R_{h+2}}$, $z\in K\cap B_{R_{h+1}}$ be a point of minimal distance, and suppose that $z\in K\setminus K_h$. 
Being $R_{h+1}\leq S_h$, by the very definition of $K_h$ there is a ball 
$B\in\cup_{j=1}^h \mathcal{F}_j$ such that $z\in B$. In turn, since $B=B_\rho(y)$ for some $y$ and radius $\rho\geq t\,M^{-h}$, then $x\in B_{2t}(y)$ as $|x-z|\leq M^{-(h+1)}$ for $M$ sufficiently large. 
Thus, estimate $|\nabla u(x)|^2<M^{h+1}$ follows from \eqref{e:gradbdd} in item (ii) of Proposition~\ref{p:alfpor}. 
This is in contradiction with $x\in A_{h+2}$.
\end{proof}

